ExeWorldBench: Benchmarking Code-Based Executable 3D World Modeling

Coding agents are increasingly evolving beyond reproducing what a world looks like toward constructing executable worlds that capture how a world works. This shift calls for executable world modeling, which integrates two core capabilities: world understanding, reasoning about the underlying structural, mechanical, and causal principles of a world, and executable realization, translating that understanding into a code-based system whose behavior emerges from physical interactions. However, existing benchmarks provide only fragmented evaluations centered on physical reasoning, visual fidelity, or behavioral correctness, leaving the integration of these capabilities insufficiently assessed. To bridge this gap, we introduce ExeWorldBench, to our knowledge the first benchmark to comprehensively evaluate world understanding and executable realization through code-based 3D world construction. ExeWorldBench comprises three progressively challenging tasks: Mechanism Executability, which evaluates the realization of individual mechanisms from visual observations; Compositional Executability, which extends to multi-stage systems with spatial, mechanical, and causal dependencies; and Intent-Driven Executable World Synthesis, which requires constructing executable worlds from high-level goals and physical requirements. Extensive experiments on frontier models reveal substantial limitations in executable world modeling, offering insights into the development of more physically grounded and causally coherent world construction systems.

==> table/benchmark-tables.tex <==
\begin{table}[!htbp]
\centering
\caption{Results on T1-normal.}
\label{tab:t1}
\begingroup
\BTSetup{6}
\begin{tabular}{@{}>{\raggedright\arraybackslash}m{\BTmodelwidth}*{6}{>{\centering\arraybackslash}m{\BTbarwidth}}@{}}
\toprule
\multirow[c]{2}{\BTmodelwidth}[-\dimexpr(\aboverulesep+\belowrulesep+\cmidrulewidth)/2\relax]{\centering\textbf{Model}}
& \multicolumn{2}{c}{$E \uparrow$}
& \multicolumn{2}{c}{$V \uparrow$}
& \multicolumn{2}{c}{$M \uparrow$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& $E_1$ & $E_2$
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4 \\
\midrule
\BTModel{openai}{GPT-6 Astra (Codex CLI)}{\cite{openai2026gpt6astra,openai_codex_cli}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTVisual}{7.16}{10}{\textbf{7.16}}
& \BTBar{BTVisual}{7.16}{10}{\textbf{7.16}}
& \BTBar{BTMotion}{6.32}{10}{\textbf{6.32}}
& \BTBar{BTMotion}{6.32}{10}{\textbf{6.32}} \\
\BTModel{claude}{Claude Fable 5.1 (Claude Code)}{\cite{anthropic2026fable51,anthropic_claude_code}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTVisual}{6.44}{10}{6.44}
& \BTBar{BTVisual}{6.44}{10}{6.44}
& \BTBar{BTMotion}{5.68}{10}{5.68}
& \BTBar{BTMotion}{5.68}{10}{5.68} \\
\addlinespace[3pt]
\BTModel{bytedance}{Doubao-Seed-2.1-Pro}{\cite{bytedanceseed2026seed21}}
& \BTBar{BTExec}{8.00}{100}{8.00\%}
& \BTBar{BTExec}{82.00}{100}{82.00\%}
& \BTBar{BTVisual}{0.30}{10}{0.30}
& \BTBar{BTVisual}{2.16}{10}{2.16}
& \BTBar{BTMotion}{0.20}{10}{0.20}
& \BTBar{BTMotion}{1.04}{10}{1.04} \\
\BTModel{openai}{GPT-6 Astra}{\cite{openai2026gpt6astra}}
& \BTBar{BTExec}{58.00}{100}{58.00\%}
& \BTBar{BTExec}{94.00}{100}{94.00\%}
& \BTBar{BTVisual}{3.58}{10}{3.58}
& \BTBar{BTVisual}{5.84}{10}{5.84}
& \BTBar{BTMotion}{3.14}{10}{3.14}
& \BTBar{BTMotion}{5.08}{10}{5.08} \\
\BTModel{deepseek}{DeepSeek-V4.1-Flash}{\cite{deepseekai2026deepseekv41flash}}
& \BTBar{BTExec}{14.00}{100}{14.00\%}
& \BTBar{BTExec}{82.00}{100}{82.00\%}
& \BTBar{BTVisual}{0.24}{10}{0.24}
& \BTBar{BTVisual}{1.76}{10}{1.76}
& \BTBar{BTMotion}{0.08}{10}{0.08}
& \BTBar{BTMotion}{0.78}{10}{0.78} \\
\BTModel{qwen}{Qwen3.8-Max}{\cite{alibaba2026qwen38max}}
& \BTBar{BTExec}{20.00}{100}{20.00\%}
& \BTBar{BTExec}{82.00}{100}{82.00\%}
& \BTBar{BTVisual}{0.34}{10}{0.34}
& \BTBar{BTVisual}{1.34}{10}{1.34}
& \BTBar{BTMotion}{0.18}{10}{0.18}
& \BTBar{BTMotion}{0.82}{10}{0.82} \\
\BTModel{kimi}{Kimi K3}{\cite{kimiteam2026kimik3}}
& \BTBar{BTExec}{8.00}{100}{8.00\%}
& \BTBar{BTExec}{86.00}{100}{86.00\%}
& \BTBar{BTVisual}{0.12}{10}{0.12}
& \BTBar{BTVisual}{1.64}{10}{1.64}
& \BTBar{BTMotion}{0.04}{10}{0.04}
& \BTBar{BTMotion}{0.80}{10}{0.80} \\
\BTModel{zai}{GLM-5.3-Flash}{\cite{glm5team2026glm5}}
& \BTBar{BTExec}{26.00}{100}{26.00\%}
& \BTBar{BTExec}{78.00}{100}{78.00\%}
& \BTBar{BTVisual}{0.48}{10}{0.48}
& \BTBar{BTVisual}{1.52}{10}{1.52}
& \BTBar{BTMotion}{0.24}{10}{0.24}
& \BTBar{BTMotion}{0.84}{10}{0.84} \\
\BTModel{claude}{Claude Fable 5.1}{\cite{anthropic2026fable51}}
& \BTBar{BTExec}{18.00}{100}{18.00\%}
& \BTBar{BTExec}{100.00}{100}{\textbf{100.00\%}}
& \BTBar{BTVisual}{0.76}{10}{0.76}
& \BTBar{BTVisual}{4.04}{10}{4.04}
& \BTBar{BTMotion}{0.50}{10}{0.50}
& \BTBar{BTMotion}{3.24}{10}{3.24} \\
\bottomrule
\end{tabular}
\endgroup
\end{table}

\begin{table}[!htbp]
\centering
\caption{Results on T2-normal.}
\label{tab:t2}
\begingroup
\BTSetup{6}
\begin{tabular}{@{}>{\raggedright\arraybackslash}m{\BTmodelwidth}*{6}{>{\centering\arraybackslash}m{\BTbarwidth}}@{}}
\toprule
\multirow[c]{2}{\BTmodelwidth}[-\dimexpr(\aboverulesep+\belowrulesep+\cmidrulewidth)/2\relax]{\centering\textbf{Model}}
& \multicolumn{2}{c}{$E \uparrow$}
& \multicolumn{2}{c}{$V \uparrow$}
& \multicolumn{2}{c}{$\mathrm{ECM} \uparrow$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& $E_1$ & $E_2$
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4 \\
\midrule
\BTModel{openai}{GPT-6 Astra (Codex CLI)}{\cite{openai2026gpt6astra,openai_codex_cli}}
& \BTBar{BTExec}{99}{100}{99\%}
& \BTBar{BTExec}{99}{100}{99\%}
& \BTBar{BTVisual}{5.33}{10}{\textbf{5.33}}
& \BTBar{BTVisual}{5.33}{10}{\textbf{5.33}}
& \BTBar{BTMotion}{5.25}{10}{\textbf{5.25}}
& \BTBar{BTMotion}{5.25}{10}{\textbf{5.25}} \\
\BTModel{claude}{Claude Fable 5.1 (Claude Code)}{\cite{anthropic2026fable51,anthropic_claude_code}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTVisual}{4.45}{10}{4.45}
& \BTBar{BTVisual}{4.45}{10}{4.45}
& \BTBar{BTMotion}{4.08}{10}{4.08}
& \BTBar{BTMotion}{4.08}{10}{4.08} \\
\addlinespace[3pt]
\BTModel{bytedance}{Doubao-Seed-2.1-Pro}{\cite{bytedanceseed2026seed21}}
& \BTBar{BTExec}{2.00}{100}{2.00\%}
& \BTBar{BTExec}{73.00}{100}{73.00\%}
& \BTBar{BTVisual}{0.04}{10}{0.04}
& \BTBar{BTVisual}{1.12}{10}{1.12}
& \BTBar{BTMotion}{0.00}{10}{0.00}
& \BTBar{BTMotion}{0.01}{10}{0.01} \\
\BTModel{openai}{GPT-6 Astra}{\cite{openai2026gpt6astra}}
& \BTBar{BTExec}{81.00}{100}{81.00\%}
& \BTBar{BTExec}{91.00}{100}{91.00\%}
& \BTBar{BTVisual}{3.46}{10}{3.46}
& \BTBar{BTVisual}{3.86}{10}{3.86}
& \BTBar{BTMotion}{2.23}{10}{2.23}
& \BTBar{BTMotion}{2.47}{10}{2.47} \\
\BTModel{deepseek}{DeepSeek-V4.1-Flash}{\cite{deepseekai2026deepseekv41flash}}
& \BTBar{BTExec}{2.00}{100}{2.00\%}
& \BTBar{BTExec}{88.00}{100}{88.00\%}
& \BTBar{BTVisual}{0.05}{10}{0.05}
& \BTBar{BTVisual}{1.83}{10}{1.83}
& \BTBar{BTMotion}{0.00}{10}{0.00}
& \BTBar{BTMotion}{0.09}{10}{0.09} \\
\BTModel{qwen}{Qwen3.8-Max}{\cite{alibaba2026qwen38max}}
& \BTBar{BTExec}{9.00}{100}{9.00\%}
& \BTBar{BTExec}{62.00}{100}{62.00\%}
& \BTBar{BTVisual}{0.06}{10}{0.06}
& \BTBar{BTVisual}{1.21}{10}{1.21}
& \BTBar{BTMotion}{0.00}{10}{0.00}
& \BTBar{BTMotion}{0.00}{10}{0.00} \\
\BTModel{kimi}{Kimi K3}{\cite{kimiteam2026kimik3}}
& \BTBar{BTExec}{10.00}{100}{10.00\%}
& \BTBar{BTExec}{79.00}{100}{79.00\%}
& \BTBar{BTVisual}{0.19}{10}{0.19}
& \BTBar{BTVisual}{1.62}{10}{1.62}
& \BTBar{BTMotion}{0.00}{10}{0.00}
& \BTBar{BTMotion}{0.00}{10}{0.00} \\
\BTModel{zai}{GLM-5.3-Flash}{\cite{glm5team2026glm5}}
& \BTBar{BTExec}{22.00}{100}{22.00\%}
& \BTBar{BTExec}{79.00}{100}{79.00\%}
& \BTBar{BTVisual}{0.55}{10}{0.55}
& \BTBar{BTVisual}{1.97}{10}{1.97}
& \BTBar{BTMotion}{0.07}{10}{0.07}
& \BTBar{BTMotion}{0.15}{10}{0.15} \\
\BTModel{claude}{Claude Fable 5.1}{\cite{anthropic2026fable51}}
& \BTBar{BTExec}{91.00}{100}{91.00\%}
& \BTBar{BTExec}{93.00}{100}{93.00\%}
& \BTBar{BTVisual}{3.42}{10}{3.42}
& \BTBar{BTVisual}{3.49}{10}{3.49}
& \BTBar{BTMotion}{1.83}{10}{1.83}
& \BTBar{BTMotion}{1.84}{10}{1.84} \\
\bottomrule
\end{tabular}
\endgroup
\end{table}

\begin{table}[!htbp]
\centering
\caption{Results on T3-task1.}
\label{tab:t3-1}
\begingroup
\BTSetup{6}
\begin{tabular}{@{}>{\raggedright\arraybackslash}m{\BTmodelwidth}*{6}{>{\centering\arraybackslash}m{\BTbarwidth}}@{}}
\toprule
\multirow[c]{2}{\BTmodelwidth}[-\dimexpr(\aboverulesep+\belowrulesep+\cmidrulewidth)/2\relax]{\centering\textbf{Model}}
& \multicolumn{2}{c}{$E \uparrow$}
& \multicolumn{2}{c}{$V \uparrow$}
& \multicolumn{2}{c}{$\mathrm{ECM} \uparrow$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}
& $E_1$ & $E_2$
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4 \\
\midrule
\BTModel{openai}{GPT-6 Astra (Codex CLI)}{\cite{openai2026gpt6astra,openai_codex_cli}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTVisual}{5.67}{10}{\textbf{5.67}}
& \BTBar{BTVisual}{5.67}{10}{\textbf{5.67}}
& \BTBar{BTMotion}{6.11}{10}{\textbf{6.11}}
& \BTBar{BTMotion}{6.11}{10}{\textbf{6.11}} \\
\BTModel{claude}{Claude Fable 5.1 (Claude Code)}{\cite{anthropic2026fable51,anthropic_claude_code}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTVisual}{5.21}{10}{5.21}
& \BTBar{BTVisual}{5.21}{10}{5.21}
& \BTBar{BTMotion}{5.70}{10}{5.70}
& \BTBar{BTMotion}{5.70}{10}{5.70} \\
\addlinespace[3pt]
\BTModel{bytedance}{Doubao-Seed-2.1-Pro}{\cite{bytedanceseed2026seed21}}
& \BTBar{BTExec}{9.52}{100}{9.52\%}
& \BTBar{BTExec}{84.13}{100}{84.13\%}
& \BTBar{BTVisual}{0.33}{10}{0.33}
& \BTBar{BTVisual}{2.24}{10}{2.24}
& \BTBar{BTMotion}{0.05}{10}{0.05}
& \BTBar{BTMotion}{0.13}{10}{0.13} \\
\BTModel{openai}{GPT-6 Astra}{\cite{openai2026gpt6astra}}
& \BTBar{BTExec}{44.44}{100}{44.44\%}
& \BTBar{BTExec}{85.71}{100}{85.71\%}
& \BTBar{BTVisual}{2.22}{10}{2.22}
& \BTBar{BTVisual}{4.08}{10}{4.08}
& \BTBar{BTMotion}{1.83}{10}{1.83}
& \BTBar{BTMotion}{3.34}{10}{3.34} \\
\BTModel{deepseek}{DeepSeek-V4.1-Flash}{\cite{deepseekai2026deepseekv41flash}}
& \BTBar{BTExec}{4.76}{100}{4.76\%}
& \BTBar{BTExec}{87.30}{100}{87.30\%}
& \BTBar{BTVisual}{0.10}{10}{0.10}
& \BTBar{BTVisual}{2.11}{10}{2.11}
& \BTBar{BTMotion}{0.07}{10}{0.07}
& \BTBar{BTMotion}{0.29}{10}{0.29} \\
\BTModel{qwen}{Qwen3.8-Max}{\cite{alibaba2026qwen38max}}
& \BTBar{BTExec}{0.00}{100}{0.00\%}
& \BTBar{BTExec}{84.13}{100}{84.13\%}
& \BTBar{BTVisual}{0.00}{10}{0.00}
& \BTBar{BTVisual}{1.62}{10}{1.62}
& \BTBar{BTMotion}{0.00}{10}{0.00}
& \BTBar{BTMotion}{0.03}{10}{0.03} \\
\BTModel{kimi}{Kimi K3}{\cite{kimiteam2026kimik3}}
& \BTBar{BTExec}{6.35}{100}{6.35\%}
& \BTBar{BTExec}{95.24}{100}{95.24\%}
& \BTBar{BTVisual}{0.17}{10}{0.17}
& \BTBar{BTVisual}{2.37}{10}{2.37}
& \BTBar{BTMotion}{0.01}{10}{0.01}
& \BTBar{BTMotion}{0.40}{10}{0.40} \\
\BTModel{zai}{GLM-5.3-Flash}{\cite{glm5team2026glm5}}
& \BTBar{BTExec}{20.63}{100}{20.63\%}
& \BTBar{BTExec}{71.43}{100}{71.43\%}
& \BTBar{BTVisual}{0.67}{10}{0.67}
& \BTBar{BTVisual}{2.33}{10}{2.33}
& \BTBar{BTMotion}{0.10}{10}{0.10}
& \BTBar{BTMotion}{0.39}{10}{0.39} \\
\BTModel{claude}{Claude Fable 5.1}{\cite{anthropic2026fable51}}
& \BTBar{BTExec}{98.41}{100}{98.41\%}
& \BTBar{BTExec}{100.00}{100}{\textbf{100.00\%}}
& \BTBar{BTVisual}{4.32}{10}{4.32}
& \BTBar{BTVisual}{4.38}{10}{4.38}
& \BTBar{BTMotion}{2.73}{10}{2.73}
& \BTBar{BTMotion}{2.75}{10}{2.75} \\
\bottomrule
\end{tabular}
\endgroup
\end{table}

\begin{table}[!htbp]
\centering
\caption{Results on T3-task2.}
\label{tab:t3-2}
\begingroup
\BTSetup{8}
\begin{tabular}{@{}>{\raggedright\arraybackslash}m{\BTmodelwidth}*{8}{>{\centering\arraybackslash}m{\BTbarwidth}}@{}}
\toprule
\multirow[c]{2}{\BTmodelwidth}[-\dimexpr(\aboverulesep+\belowrulesep+\cmidrulewidth)/2\relax]{\centering\textbf{Model}}
& \multicolumn{2}{c}{$E \uparrow$}
& \multicolumn{2}{c}{$V \uparrow$}
& \multicolumn{2}{c}{$\mathrm{ECM} \uparrow$}
& \multicolumn{2}{c}{Goal satisfaction $\uparrow$} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}\cmidrule(lr){6-7}\cmidrule(lr){8-9}
& $E_1$ & $E_2$
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4 \\
\midrule
\BTModel{openai}{GPT-6 Astra (Codex CLI)}{\cite{openai2026gpt6astra,openai_codex_cli}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTVisual}{6.28}{10}{\textbf{6.28}}
& \BTBar{BTVisual}{6.28}{10}{\textbf{6.28}}
& \BTBar{BTMotion}{5.82}{10}{\textbf{5.82}}
& \BTBar{BTMotion}{5.82}{10}{\textbf{5.82}}
& \BTBar{BTGoal}{90.14}{100}{\textbf{90.14\%}}
& \BTBar{BTGoal}{90.14}{100}{\textbf{90.14\%}} \\
\BTModel{claude}{Claude Fable 5.1 (Claude Code)}{\cite{anthropic2026fable51,anthropic_claude_code}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTExec}{100}{100}{\textbf{100\%}}
& \BTBar{BTVisual}{5.83}{10}{5.83}
& \BTBar{BTVisual}{5.83}{10}{5.83}
& \BTBar{BTMotion}{5.17}{10}{5.17}
& \BTBar{BTMotion}{5.17}{10}{5.17}
& \BTBar{BTGoal}{75.19}{100}{75.19\%}
& \BTBar{BTGoal}{75.19}{100}{75.19\%} \\
\addlinespace[3pt]
\BTModel{bytedance}{Doubao-Seed-2.1-Pro}{\cite{bytedanceseed2026seed21}}
& \BTBar{BTExec}{1.67}{100}{1.67\%}
& \BTBar{BTExec}{70.00}{100}{70.00\%}
& \BTBar{BTVisual}{0.05}{10}{0.05}
& \BTBar{BTVisual}{1.82}{10}{1.82}
& \BTBar{BTMotion}{0.02}{10}{0.02}
& \BTBar{BTMotion}{0.33}{10}{0.33}
& \BTBar{BTGoal}{0.26}{100}{0.26\%}
& \BTBar{BTGoal}{7.48}{100}{7.48\%} \\
\BTModel{openai}{GPT-6 Astra}{\cite{openai2026gpt6astra}}
& \BTBar{BTExec}{40.00}{100}{40.00\%}
& \BTBar{BTExec}{91.67}{100}{91.67\%}
& \BTBar{BTVisual}{1.97}{10}{1.97}
& \BTBar{BTVisual}{4.33}{10}{4.33}
& \BTBar{BTMotion}{1.15}{10}{1.15}
& \BTBar{BTMotion}{2.55}{10}{2.55}
& \BTBar{BTGoal}{19.17}{100}{19.17\%}
& \BTBar{BTGoal}{41.07}{100}{41.07\%} \\
\BTModel{deepseek}{DeepSeek-V4.1-Flash}{\cite{deepseekai2026deepseekv41flash}}
& \BTBar{BTExec}{10.00}{100}{10.00\%}
& \BTBar{BTExec}{81.67}{100}{81.67\%}
& \BTBar{BTVisual}{0.25}{10}{0.25}
& \BTBar{BTVisual}{1.77}{10}{1.77}
& \BTBar{BTMotion}{0.05}{10}{0.05}
& \BTBar{BTMotion}{0.52}{10}{0.52}
& \BTBar{BTGoal}{1.15}{100}{1.15\%}
& \BTBar{BTGoal}{7.52}{100}{7.52\%} \\
\BTModel{qwen}{Qwen3.8-Max}{\cite{alibaba2026qwen38max}}
& \BTBar{BTExec}{0.00}{100}{0.00\%}
& \BTBar{BTExec}{81.67}{100}{81.67\%}
& \BTBar{BTVisual}{0.00}{10}{0.00}
& \BTBar{BTVisual}{1.83}{10}{1.83}
& \BTBar{BTMotion}{0.00}{10}{0.00}
& \BTBar{BTMotion}{0.37}{10}{0.37}
& \BTBar{BTGoal}{0.00}{100}{0.00\%}
& \BTBar{BTGoal}{5.85}{100}{5.85\%} \\
\BTModel{kimi}{Kimi K3}{\cite{kimiteam2026kimik3}}
& \BTBar{BTExec}{3.33}{100}{3.33\%}
& \BTBar{BTExec}{81.67}{100}{81.67\%}
& \BTBar{BTVisual}{0.13}{10}{0.13}
& \BTBar{BTVisual}{2.70}{10}{2.70}
& \BTBar{BTMotion}{0.05}{10}{0.05}
& \BTBar{BTMotion}{0.63}{10}{0.63}
& \BTBar{BTGoal}{1.53}{100}{1.53\%}
& \BTBar{BTGoal}{18.13}{100}{18.13\%} \\
\BTModel{zai}{GLM-5.3-Flash}{\cite{glm5team2026glm5}}
& \BTBar{BTExec}{10.00}{100}{10.00\%}
& \BTBar{BTExec}{30.00}{100}{30.00\%}
& \BTBar{BTVisual}{0.32}{10}{0.32}
& \BTBar{BTVisual}{1.07}{10}{1.07}
& \BTBar{BTMotion}{0.00}{10}{0.00}
& \BTBar{BTMotion}{0.15}{10}{0.15}
& \BTBar{BTGoal}{0.86}{100}{0.86\%}
& \BTBar{BTGoal}{5.29}{100}{5.29\%} \\
\BTModel{claude}{Claude Fable 5.1}{\cite{anthropic2026fable51}}
& \BTBar{BTExec}{73.33}{100}{73.33\%}
& \BTBar{BTExec}{78.33}{100}{78.33\%}
& \BTBar{BTVisual}{3.22}{10}{3.22}
& \BTBar{BTVisual}{3.47}{10}{3.47}
& \BTBar{BTMotion}{1.68}{10}{1.68}
& \BTBar{BTMotion}{1.85}{10}{1.85}
& \BTBar{BTGoal}{28.83}{100}{28.83\%}
& \BTBar{BTGoal}{31.31}{100}{31.31\%} \\
\bottomrule
\end{tabular}
\endgroup
\end{table}


==> table/model-icons/benchmark-table-style.tex <==
% Load once in the preamble. No shell escape or SVG converter is needed.
\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{array}
\usepackage{multirow}
\usepackage{xcolor}
\usepackage{tikz}
\usepackage{etoolbox}

\definecolor{BTExec}{HTML}{A998ED}
\definecolor{BTVisual}{HTML}{EDB75D}
\definecolor{BTMotion}{HTML}{68AEA5}
\definecolor{BTGoal}{HTML}{A998ED}

\newlength{\BTmodelwidth}
\newlength{\BTbarwidth}
\newcommand{\BTiconpath}{model-icons}

% #1 = metric column count. All columns fit the current linewidth,
% without shrinking the entire table (including model labels/citations).
\newcommand{\BTSetup}[1]{%
  \fontsize{8.5pt}{10.5pt}\selectfont
  \setlength{\tabcolsep}{2pt}%
  \renewcommand{\arraystretch}{1.10}%
  \setlength{\extrarowheight}{2pt}%
  \ifnum#1=8
    \setlength{\BTmodelwidth}{0.32\linewidth}%
  \else
    \setlength{\BTmodelwidth}{0.36\linewidth}%
  \fi
  \setlength{\BTbarwidth}{%
    \dimexpr(\linewidth-\BTmodelwidth-\tabcolsep*2*#1)/#1\relax}%
}

\newcommand{\BTIcon}[1]{%
  \IfFileExists{\BTiconpath/#1.png}{%
    \raisebox{-0.18em}{%
      \includegraphics[width=1.15em,height=1.15em,keepaspectratio]{\BTiconpath/#1.png}}%
  }{%
    \PackageWarning{benchmark-tables}{Missing icon: \BTiconpath/#1.png}%
    \makebox[1.15em]{\textbullet}%
  }%
}

% Provider icon, original model name, original citation.
\newcommand{\BTModel}[3]{%
  \BTIcon{#1}\hspace{0.35em}#2\par
  {\fontsize{6.5pt}{8pt}\selectfont #3\par}%
}

% #1 color; #2 numeric value or "-"; #3 fixed maximum; #4 printed label.
% Missing data are not zero. Zero has only the faint background, no fill.
\newcommand{\BTBar}[4]{%
  \ifstrequal{#2}{-}{%
    \makebox[\BTbarwidth][c]{-}%
  }{%
    \begingroup
    \pgfmathsetmacro{\BTfraction}{max(0,min(1,(#2)/(#3)))}%
    \begin{tikzpicture}[x=\BTbarwidth,y=14pt,baseline=(BTvalue.base)]
      \path[use as bounding box] (0,0) rectangle (1,1);
      \begin{scope}
        \clip[rounded corners=1.2pt] (0,0) rectangle (1,1);
        \fill[#1!15!white] (0,0) rectangle (1,1);
        \ifdim\BTfraction pt>0pt
          \shade[left color=#1!85!white,right color=#1!48!white]
            (0,0) rectangle (\BTfraction,1);
        \fi
      \end{scope}
      \node[inner sep=0pt,outer sep=0pt,
        font=\normalfont\fontsize{8pt}{9pt}\selectfont]
        (BTvalue) at (0.5,0.5) {#4};
    \end{tikzpicture}%
    \endgroup
  }%
}


==> table/original-tables.tex <==
\begin{table}[!htbp]
\centering
\caption{Results on T1-normal.}
\label{tab:t1}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{$E \uparrow$}
& \multicolumn{2}{c}{$V \uparrow$}
& \multicolumn{2}{c}{$M \uparrow$} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
Model
& $E_1$ & $E_2$
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4 \\
\midrule
GPT-6 Astra (Codex CLI)~ \cite{openai2026gpt6astra,openai_codex_cli}
& 100\% & 100\% & 7.16 & 7.16 & 6.32 & 6.32 \\
Claude Fable 5.1 (Claude Code)~ \cite{anthropic2026fable51,anthropic_claude_code}
& 100\% & 100\% & 6.44 & 6.44 & 5.68 & 5.68 \\
Doubao-Seed-2.1-Pro~\cite{bytedanceseed2026seed21}
& 8.00\% & 82.00\% & 0.30 & 2.16 & 0.20 & 1.04 \\
GPT-6 Astra~\cite{openai2026gpt6astra}
& 58.00\% & 94.00\% & 3.58 & 5.84 & 3.14 & 5.08 \\
DeepSeek-V4.1-Flash~\cite{deepseekai2026deepseekv41flash}
& 14.00\% & 82.00\% & 0.24 & 1.76 & 0.08 & 0.78 \\
Qwen3.8-Max~\cite{alibaba2026qwen38max}
& 20.00\% & 82.00\% & 0.34 & 1.34 & 0.18 & 0.82 \\
Kimi K3~\cite{kimiteam2026kimik3}
& 8.00\% & 86.00\% & 0.12 & 1.64 & 0.04 & 0.80 \\
GLM-5.3-Flash~\cite{glm5team2026glm5}
& 26.00\% & 78.00\% & 0.48 & 1.52 & 0.24 & 0.84 \\
Claude Fable 5.1~\cite{anthropic2026fable51}
& 18.00\% & 100.00\% & 0.76 & 4.04 & 0.50 & 3.24 \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[!htbp]
\centering
\caption{Results on T2-normal.}
\label{tab:t2}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{$E \uparrow$}
& \multicolumn{2}{c}{$V \uparrow$}
& \multicolumn{2}{c}{$\mathrm{ECM} \uparrow$} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
Model
& $E_1$ & $E_2$
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4 \\
\midrule
GPT-6 Astra (Codex CLI)~ \cite{openai2026gpt6astra,openai_codex_cli}
& 99\% & 99\% & 5.33 & 5.33 & 5.25 & 5.25 \\
Claude Fable 5.1 (Claude Code)~ \cite{anthropic2026fable51,anthropic_claude_code}
& 100\% & 100\% & 4.45 & 4.45 & 4.08 & 4.08 \\
Doubao-Seed-2.1-Pro~\cite{bytedanceseed2026seed21}
& 2.00\% & 73.00\% & 0.04 & 1.12 & 0.00 & 0.01 \\
GPT-6 Astra~\cite{openai2026gpt6astra}
& 81.00\% & 91.00\% & 3.46 & 3.86 & 2.23 & 2.47 \\
DeepSeek-V4.1-Flash~\cite{deepseekai2026deepseekv41flash}
& 2.00\% & 88.00\% & 0.05 & 1.83 & 0.00 & 0.09 \\
Qwen3.8-Max~\cite{alibaba2026qwen38max}
& 9.00\% & 62.00\% & 0.06 & 1.21 & 0.00 & 0.00 \\
Kimi K3~\cite{kimiteam2026kimik3}
& 10.00\% & 79.00\% & 0.19 & 1.62 & 0.00 & 0.00 \\
GLM-5.3-Flash~\cite{glm5team2026glm5}
& 22.00\% & 79.00\% & 0.55 & 1.97 & 0.07 & 0.15 \\
Claude Fable 5.1~\cite{anthropic2026fable51}
& 91.00\% & 93.00\% & 3.42 & 3.49 & 1.83 & 1.84 \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[!htbp]
\centering
\caption{Results on T3-task1.}
\label{tab:t3-1}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
& \multicolumn{2}{c}{$E \uparrow$}
& \multicolumn{2}{c}{$V \uparrow$}
& \multicolumn{2}{c}{$\mathrm{ECM} \uparrow$} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
Model
& $E_1$ & $E_2$
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4 \\
\midrule
GPT-6 Astra (Codex CLI)~ \cite{openai2026gpt6astra,openai_codex_cli}
& 100\% & 100\% & 5.67 & 5.67 & 6.11 & 6.11 \\
Claude Fable 5.1 (Claude Code)~ \cite{anthropic2026fable51,anthropic_claude_code}
& 100\% & 100\% & 5.21 & 5.21 & 5.70 & 5.70 \\
Doubao-Seed-2.1-Pro~\cite{bytedanceseed2026seed21}
& 9.52\% & 84.13\% & 0.33 & 2.24 & 0.05 & 0.13 \\
GPT-6 Astra~\cite{openai2026gpt6astra}
& 44.44\% & 85.71\% & 2.22 & 4.08 & 1.83 & 3.34 \\
DeepSeek-V4.1-Flash~\cite{deepseekai2026deepseekv41flash}
& 4.76\% & 87.30\% & 0.10 & 2.11 & 0.07 & 0.29 \\
Qwen3.8-Max~\cite{alibaba2026qwen38max}
& 0.00\% & 84.13\% & 0.00 & 1.62 & 0.00 & 0.03 \\
Kimi K3~\cite{kimiteam2026kimik3}
& 6.35\% & 95.24\% & 0.17 & 2.37 & 0.01 & 0.40 \\
GLM-5.3-Flash~\cite{glm5team2026glm5}
& 20.63\% & 71.43\% & 0.67 & 2.33 & 0.10 & 0.39 \\
Claude Fable 5.1~\cite{anthropic2026fable51}
& 98.41\% & 100.00\% & 4.32 & 4.38 & 2.73 & 2.75 \\
\bottomrule
\end{tabular}%
}
\end{table}

\begin{table}[!htbp]
\centering
\caption{Results on T3-task2.}
\label{tab:t3-2}
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccccc}
\toprule
& \multicolumn{2}{c}{$E \uparrow$}
& \multicolumn{2}{c}{$V \uparrow$}
& \multicolumn{2}{c}{$\mathrm{ECM} \uparrow$}
& \multicolumn{2}{c}{Goal satisfaction $\uparrow$} \\
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
\cmidrule(lr){8-9}
Model
& $E_1$ & $E_2$
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4
& Alg.~2 & Alg.~4 \\
\midrule
GPT-6 Astra (Codex CLI)~ \cite{openai2026gpt6astra,openai_codex_cli}
& 100\% & 100\% & 6.28 & 6.28 & 5.82 & 5.82 & 90.14\% & 90.14\% \\
Claude Fable 5.1 (Claude Code)~ \cite{anthropic2026fable51,anthropic_claude_code}
& 100\% & 100\% & 5.83 & 5.83 & 5.17 & 5.17 & 75.19\% & 75.19\% \\
Doubao-Seed-2.1-Pro~\cite{bytedanceseed2026seed21}
& 1.67\% & 70.00\% & 0.05 & 1.82 & 0.02 & 0.33 & 0.26\% & 7.48\% \\
GPT-6 Astra~\cite{openai2026gpt6astra}
& 40.00\% & 91.67\% & 1.97 & 4.33 & 1.15 & 2.55 & 19.17\% & 41.07\% \\
DeepSeek-V4.1-Flash~\cite{deepseekai2026deepseekv41flash}
& 10.00\% & 81.67\% & 0.25 & 1.77 & 0.05 & 0.52 & 1.15\% & 7.52\% \\
Qwen3.8-Max~\cite{alibaba2026qwen38max}
& 0.00\% & 81.67\% & 0.00 & 1.83 & 0.00 & 0.37 & 0.00\% & 5.85\% \\
Kimi K3~\cite{kimiteam2026kimik3}
& 3.33\% & 81.67\% & 0.13 & 2.70 & 0.05 & 0.63 & 1.53\% & 18.13\% \\
GLM-5.3-Flash~\cite{glm5team2026glm5}
& 10.00\% & 30.00\% & 0.32 & 1.07 & 0.00 & 0.15 & 0.86\% & 5.29\% \\
Claude Fable 5.1~\cite{anthropic2026fable51}
& 73.33\% & 78.33\% & 3.22 & 3.47 & 1.68 & 1.85 & 28.83\% & 31.31\% \\
\bottomrule
\end{tabular}%
}
\end{table}

